OCTAL: Graph Representation Learning for LTL Model Checking

Model Checking is widely applied in verifying the correctness of complex and concurrent systems against a specification. Pure symbolic approaches while popular, suffer from the state space explosion problem due to cross product operations required that make them prohibitively expensive for large-scale systems and/or specifications. In this paper, we propose to use graph representation learning (GRL) for solving linear temporal logic (LTL) model checking, where the system and the specification are expressed by a B{\"u}chi automaton and an LTL formula, respectively. A novel GRL-based framework \model, is designed to learn the representation of the graph-structured system and specification, which reduces the model checking problem to binary classification. Empirical experiments on two model checking scenarios show that \model achieves promising accuracy, with up to $11\times$ overall speedup against canonical SOTA model checkers and $31\times$ for satisfiability checking alone.

==> Preliminaries.tex <==
\section{Preliminaries \label{sec:Prelim}}
\subsection{B{\"u}chi Automata}
In automata theory, a B{\"u}chi automaton (BA) is a system that either accepts or rejects inputs of infinite length. The automaton is represented by a set of states (one initial, some final, and others neither initial nor final), a transition relation, which determines which state should the present state move to, depending on the alphabets that hold in the transition. The system accepts an input if and only if it visits at least one accepting state infinitely often for the input. A B{\"u}chi automaton can be deterministic or non-deterministic. We deal with non-deterministic B{\"u}chi automata systems in this paper, as they are strictly more powerful than deterministic B{\"u}chi automata systems.

A non-deterministic B{\"u}chi automaton $B$ is formally defined as the tuple $(Q, \sum, \Delta, q_{0}, \mathbf{q}_{f})$, where $Q$ is the set of all states of $B$, and is finite; $\sum$ is the finite set of alphabets; $\Delta: Q \times 2^{\sum} \rightarrow 2^Q$ is the transition relation that can map a state to a set of states on the same input set; $q_{0} \in Q$ represents the initial state; $\mathbf{q}_{f} \subset Q$ is the set of final states.

\subsection{Linear Temporal Logic}
Linear Temporal Logic (LTL), is a type of temporal logic that models properties with respect to time. An LTL formula is constructed from a finite set of atomic propositions, logical operators not (!), and (\&), and or ($|$), true (1), false ($N$), and temporal operators. Additional logical operators such as implies, equivalence, etc. that can be replaced by the combination of basic logical operators $(!, \&, |)$. For example, $a \rightarrow b$ is expressed as $!a \: | \: b$.

\begin{figure*}
%\centering
%\hfill
\subfigure[$B$ accepting `$a \: U \: b$'.\label{FigurelabelBASpec}]{
\begin{minipage}{0.3\textwidth}
%\centering    
\includegraphics[height=3.5cm]{tikzPDFs/fig1a.pdf}
\vspace{5mm}
\end{minipage}
}
%\hfill
\subfigure[$B_{\neg \phi}$ accepting `$!(a \: U \: b)$' \label{FigurelabelNegBASpec}]{
\begin{minipage}{0.3\textwidth}
%\centering
\includegraphics[height=3.5cm]{tikzPDFs/fig1b.pdf}
\vspace{5mm}
\end{minipage}
}
%\hfill
\subfigure[$B' = B \times B_{\neg \phi}$\label{FigurelabelBACrossProd}]{
\begin{minipage}{0.3\textwidth}
\centering
\includegraphics[height=4cm]{tikzPDFs/fig2.pdf}
\end{minipage}
}
%\vspace{-3mm}
\caption{Illustration of systems $B$, $B_{\neg \phi}$ and their product $B'$. $B$ accepts `$a \: U \: b$', meaning $a$ must be true until $b$ becomes true. $B_{\neg \phi}$ accepts `$!(a \: U \: b)$', where $\neg \phi$ is the negation of `$a \: U \: b$'. $B'$ is the cross product of $B$ and $B_{\neg \phi}$, which significantly increases the state size. \label{fig:prod}}
\vspace{-3mm}
\end{figure*}

\subsection{LTL Model Checking}
Given a B{\"u}chi automaton $B$ (system), and an LTL formula $\phi$ (specification), the model checking problem decides whether $B$ satisfies  $\phi$. Traditionally, the problem is solved by computing the B{\"u}chi automaton for the negation of the specification $\phi$ as $B_{\neg \phi}$, followed by the product automaton $B' = B \times B_{\neg \phi}$. The problem then reduces to checking the language emptiness of $B'$. The language accepted by $B'$ is said to be empty if and only if $B'$ rejects all inputs. Construction of $B$ is linear in the size of its state space, while $B_{\neg \phi}$ is exponential in the size of $\neg \phi$. The product construction would also lead to an automaton of size $|B| \times 2^{|\neg \phi|}$, which can blow up even $\phi$ is linear in the size of $B$, leading to the state space explosion problem. Figure \ref{FigurelabelBASpec} represents the system $B$ with $\phi$: `$a \: U \: b$', and Figure \ref{FigurelabelNegBASpec} represents $B_{\neg \phi}$. The cross product $B'=B\times B_{\neg \phi}$ is given in Figure \ref{FigurelabelBACrossProd}. $B'$ does not accept anything as there is no feasible path from the initial state ($q'_{0}q_{0}$) to either of the final states ($q'_{0}q_{f}$, $q'_{f}q_{f}$). Here, both $B$ and $B_{\neg \phi}$ are three times smaller than $B'$ in terms of the number of states, and 6 times smaller regarding the number of transitions. As observed in Figure \ref{fig:prod}, it can be concluded that even for moderately complex specifications, the product can still result in an exponential state space, which would severely hinder the performance of traditional model checkers.
%The system $B$ accepting `$a \: U \: b$`, which means that $a$ must be true until $b$ becomes true
%The system $B_{\neg \phi}$ accepting `$!(a \: U \: b)$`, where $\phi$ is `$a \: U \: b$`

\subsection{Graph Neural Networks}
Graph Neural Networks (GNN) extend regular neural networks to better support representation learning in graph domains. A GNN takes the input formed as a graph $\mathcal{G} = (\mathcal{V},\mathcal{E})$, where $\mathcal{V}=[n]$ represents the node set and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ is the edge set. The graph can be directed or undirected. Each node $v \in \mathcal{V}$ can be associated with node attributes as $X_v \in \mathbb{R}^{d_v}$. Similarly, each edge $e_{ij}:(v_i, v_j) \in \mathcal{E}$ can also have attributes noted as $E_{ij} \in \mathbb{R}^{d_e}$. Here, $d_v$ and $d_e$ are dimension of node features and edge features, respectively. 

GNNs aim to learn a vector representation $\mathbf{h}_v$ for each node $v$ by aggregating the neighbourhood information and iteratively updating its own hidden representation through $k$ hops as
\[\mathbf{h}_v^k=\text{UPDATE}\left(\mathbf{h}_v^{k-1}, \text{AGGREGATE}\left(\{\mathbf{h}_u^{k-1}|u\in \mathcal{N}_v\}\right)\right).\] 
Here, UPDATE is implemented by neural networks while AGGREGATE is a pooling operation that is invariant to the permutation of the neighbors $\mathcal{N}_v$ regarding node $v$. GNNs combine structural information and node features via message passing on the given graph $\mathcal{G}$. In contrast to standard neural networks, it has the capacity to retain the node representation captured by propagation up to any depth. Recently, GNNs have achieved groundbreaking success on tasks with graph-structured data, especially in node classification \cite{kipf2016semi,hamilton2017inductive,velivckovic2017graph} and graph classification \cite{xu2018powerful,GNNGraphClass}. This motivates us to exploit the structural property of $B$ and  $\phi$, and then represent them as graphs for classification, where the goal is to determine whether $B$ satisfies $\phi$ or not.
%\vspace{-3mm}
